GePA*SE: Generalized Edge-Based Parallel A* for Slow Evaluations

Parallel search algorithms have been shown to improve planning speed by harnessing the multithreading capability of modern processors. One such algorithm PA*SE achieves this by parallelizing state expansions, whereas another algorithm ePA*SE achieves this by effectively parallelizing edge evaluations. ePA*SE targets domains in which the action space comprises actions with expensive but similar evaluation times. However, in a number of robotics domains, the action space is heterogenous in the computational effort required to evaluate the cost of an action and its outcome. Motivated by this, we introduce GePA*SE: Generalized Edge-based Parallel A* for Slow Evaluations, which generalizes the key ideas of PA*SE and ePA*SE i.e. parallelization of state expansions and edge evaluations respectively. This extends its applicability to domains that have actions requiring varying computational effort to evaluate them. The open-source code for GePA*SE along with the baselines is available here: https://github.com/shohinm/parallel_search

==> 04problem.tex <==
Let a finite graph $\graph = (\Vertices, \Edges)$ be defined as a set of vertices \Vertices and directed edges \Edges. Each vertex $\vertex \in \Vertices$ represents a state \state in the state space of the domain \States. An edge $\ed \in \Edges$ connecting two vertices $\vertex_1$ and $\vertex_2$ in the graph represents an action $\ac \in \Aset$ that takes the agent from corresponding state $\state_1$ to $\state_2$. The action space is split into subsets of cheap (\Asetcheap) and expensive actions (\Asetexp) s.t. $\Asetcheap\cup\Asetexp = \Aset$ and corresponding cheap (\Edgescheap) and expensive edges (\Edgesexp) s.t. $\Edgescheap\cup\Edgesexp=\Edges$. An edge \ed can be represented as a pair \edge, where \state is the state at which action \ac is executed. For an edge \ed, we will refer to the corresponding state and action as $\ed.\state$ and $\ed.\ac$ respectively. \startstate is the start state and \goalreg is the goal region. $\cost:\Edges \rightarrow [0,\infty]$ is the cost associated with an edge. $\gval(\state)$ or g-value is the cost of the best path to \state from \startstate found by the algorithm so far. $\hval(\state)$ is a consistent heuristic~\cite{russell2010artificial}. A path \plan is an ordered sequence of edges $\ed_{i=1}^N = \edge_{i=1}^N$, the cost of which is denoted as $\cost(\plan) = \sum_{i=1}^N \cost(\ed_i)$. The objective is to find a path \plan from $\state_0$ to a state in the goal region \goalreg with the optimal cost \costopt. There is a computational budget of \numthreads parallel threads available. There exists a pairwise heuristic function $\hval(\state, \state')$ that provides an estimate of the cost between any pair of states. It is forward-backward consistent~\cite{phillips2014pa} i.e. $\hval(\state, \state'') \leq \hval(\state, \state') + \hval(\state', \state'')~\forall~\state,\state',\state''$ and $\hval(\state, \state') \leq \costopt(\state, \state')~\forall~\state, \state'$.

